VisDA 2022 Challenge: Domain Adaptation for Industrial Waste Sorting

Label-efficient and reliable semantic segmentation is essential for many real-life applications, especially for industrial settings with high visual diversity, such as waste sorting. In industrial waste sorting, one of the biggest challenges is the extreme diversity of the input stream depending on factors like the location of the sorting facility, the equipment available in the facility, and the time of year, all of which significantly impact the composition and visual appearance of the waste stream. These changes in the data are called ``visual domains'', and label-efficient adaptation of models to such domains is needed for successful semantic segmentation of industrial waste. To test the abilities of computer vision models on this task, we present the VisDA 2022 Challenge on Domain Adaptation for Industrial Waste Sorting. Our challenge incorporates a fully-annotated waste sorting dataset, ZeroWaste, collected from two real material recovery facilities in different locations and seasons, as well as a novel procedurally generated synthetic waste sorting dataset, SynthWaste. In this competition, we aim to answer two questions: 1) can we leverage domain adaptation techniques to minimize the domain gap? and 2) can synthetic data augmentation improve performance on this task and help adapt to changing data distributions? The results of the competition show that industrial waste detection poses a real domain adaptation problem, that domain generalization techniques such as augmentations, ensembling, etc., improve the overall performance on the unlabeled target domain examples, and that leveraging synthetic data effectively remains an open problem. See https://ai.bu.edu/visda-2022/

==> CHANGES <==
v1.30 (2022-02-09):

  * jmlrutils.sty:

    - fixed counter name in lemma definition when cleveref option on

v1.29 (2022-01-29):

  * jmlr.cls:

    - added cleveref option

    - fixed draft option

    - bug fix #168: Float-only last pages not counted for page numbering
       https://www.dickimaw-books.com/bugtracker.php?key=168

  * jmlrutils.sty:

    - added cleveref option

    - added \jmlralgorule

    - added \jmlrminsubcaptionwidth

  * jmlrbook.cls:

    - obsoleted (https://www.dickimaw-books.com/faq.php?itemlabel=latex20201009)
      Production editors will need to set the first page number
      of each article manually.

v1.28 (2020-09-21):

  * jmlr.cls:

   Bug fixes: 

    - fixed twoside option (which should be the default)

    - \thanks now uses mpfootnote instead of footnote counter
      with matching \footnotemark and \footnotetext optional
      arguments.

v1.27 (2020-03-26):

  * jmlrutils.sty:

    Bug fix: subfigure and subtable references were producing
    extraneous text (added check for LaTeX kernel version)

v1.26 (2020-01-31):

  * jmlr.cls:

    - removed \vbox from \@jmlrmaketitle to allow for extremely long
      author/affiliation list. Added \ignorespaces before \@author
      to allow for spacing the contents in the code for clarity
      at the start of a long author list.

v1.25 (2020-01-17):

  * jmlr.cls: 

    - Added check for graphics.sty 2019/07/01 (which now detokenizes
      filename)

  * jmlrutils.sty:

    - Added \proofname

v1.24 (2017-08-01):

  * moved non-class related code into new package jmlrutils.sty

  * fixed bug in \includeteximage

v1.23 (2017-03-09):

  * added pmlr class option

v1.22 (2015-04-11):

  * added oneside and twoside class options

v1.21 (2015-02-24):

  * jmlr.cls

    - added check for jmlr2e and pseudocode

    - fixed bug in \thanks to fix footnote marker issue if there's
      more than one \thanks

  * jmlrbook.cls

    - added \nopagebreak after \@editorialteam

v1.20 (2014-10-15):

  * jmlrbook.cls

    - added \jmlrprefaceheader, \jmlrlocation

v1.19 (2014-09-29):

  * jmlrbook.cls

    - changed \chapter* to \chapter in preface environment

v1.18 (2013-10-17):

  * jmlrbook.cls

    - patched to work with auxhook

    - added draft and final options

    - add \booklinebreak

  * jmlr.cls

    - Added calc and etoolbox as required packages

    - Added draft and final options and removed \ds@draft

    - Added starred version of \newtheorem

    - Added \theorembodyfont, \theoremheaderfont, \theorempostheader
      and \theoremsep

v1.17 (2012-05-30):

  * jmlr.cls

    - added \titletag

    - added warnings if obsolete font commands (such as \bf) used

  * jmlrbook.cls

    - added 'articlet' page style

    - \importarticle sets title page style to articlet

    - \importpaper disables \jmlryear, \jmlrworkshop, \jmlrvolume
      and \jmlrissue

    - html title page uses jmlrvolume instead of volume

    - added optional argument to \logo

v1.16 (2012-05-15):

  * jmlr.cls

    - added \@post@hyperref hook

  * jmlrbook.cls

    - added code to deal with \c@lenddoca clash

v1.15 (2012-05-12):

  * jmlrbook.cls

    - added 'algocf' and 'definition' counters to reset list in
      \zeroextracounters

    - added \theHalgocf

    - removed dependence on \ps@headings in \ps@jmlrbook

    - added \markleft

v1.14 (2012-04-24):

  * jmlrbook.cls

    - modified \jmlrwritepdfinfo to write book author and title
      information to aux file
    - fixed bug in fetching time zone information

v1.13 (2012-02-25):

  * jmlrbook.cls

    - added pdfxa option
    - added \jmlrwritepdfinfo
    - changed preface environment to use \chapter* instead of \chapter

  * jmlr.cls

    - added \@pre@hyperref hook

v1.12 (2012-01-05):

  * jmlr.cls

    - removed prehyperref package option.

    - renamed \jmlr@prehyperref to \jmlrprehyperref

    - added tabularx to list of problem packages.

    - provided default value of \@shortitle

    - added \titlebreak

    - added optional argument to \Name
      (\jmlrauthors now redefines \@jmlr@authors instead of
      \@jmlrauthors)

    - added chapter number to \theHsection to ensure unique
      hyperlinks in book

  * jmlrbook.cls

    - Moved loading setspace and fink before jmlr.cls loaded

    - changed \thechapter to \theHchapter in definition of
      \theHalgorithm etc

    - added \theHfootnote, \theHtable, \theHfigure

    - in \importpubpaper etc, changed \@shortitle to \@title in toc

  * makejmlrbook v0.31

    - footnotes in abstract files changed to in-line parentheses.

    - --batchtex option now also passes "-interaction=batchmode" to
      htlatex

    - added debugging option --noexecute

v1.11 (2011-03-24):

  * jmlr.cls

    - fixed typo: WC\&P -> W\&CP

    - added \jmlrabbrnamelist (used by makejmlrbook)

  * jmlrbook.cls

    - now requires fink package

    - added preface environment and \prefacename

    - added algorithm2e old commands (in case some authors are using
      an older version).

  * makejmlrbook (v0.3):

    - added changes made by Olivier Chapelle to add JMLR menu on the
      left side of the page and use description environment for each
      paper of the TOC.

    - added --extractpreface option

    - set hyperref draft mode for abstract only html pages.

    - abstract html source files now input original aux files to allow
      for citations.

v1.10 (2011-01-05):

  jmlr.cls

  * now loads xkeyval

  * now loads hyperref (instead of jmlrbook loading it)

  * added class option prehyperref={stuff to do before hyperref loaded}

  * added class option tablecaption=<position> (where <position> can
    either be top or bottom).

  * fixed 10pt, 11pt and 12pt class options, which weren't having
    any effect.

  * modified \thanks to ensure hyperlink works correctly.

  * added \mdseries to definition of \addr.

  * added \startpage (used by jmlrmakebook).

  * modified \artpart and \bookpart to correct bookmark level number

  jmlrbook.cls

  * code loading hyperref moved to jmlr.cls

  * added 10pt, 11pt and 12pt class options.

  * Removed redundant redefinition of \@bookpart

  makejmlrbook (v0.2):

  * Uses \startpage to set initial page number for stand-alone 
    articles.

  * Makes subdirectories in html directory for each article.

  * copies any image files generated by tex4ht into html directory.

  * added time stamp at the end of each of the generated html file.

v1.09 (2010-12-01):

  jmlr.cls

  * now loads article.cls instead of scrartcl.cls

  * Fixed sub-captions so that they don't exceed the width of the
    sub-figure/table to which they refer.

  * added \nametag, \reprint, \algocfconts, \theHsubfigure,
    \booktocpreamble, \@partapp.

  * Made \objectref robust

  jmlrbook.cls

  * Reset start and end document hook to avoid problems caused by
    defining duplicate commands.

  * Moved redefinition of \jmlrpremaketitlehook outside of import
    macros.

  * Moved \refstepcounter from \jmlrmaketitlehook to
    \jmlrpremaketitlehook

  * Added \jmlrimporthook

  * Added \label to \jmlrmaketitlehook

v1.08 (2010-07-27):

  * Fixed \thanks so that the footnote symbol is raised and isn't
    followed by a full stop.

v1.07 (2010-06-30):

  * Added check for two column

v1.06 (2010-06-17):

  jmlr.cls

  * Added tablecaptiontop and tablecaptionbottom class options

v1.05:

  jmlrbook.cls

  * Added \productioneditors

v1.04:

  * Added Perl script makejmlrbook

  jmlrbook.cls

  * Added patch to fix references in print mode

  * Added code to work with makejmlrbook

  jmlr.cls

  * Added code to work with makejmlrbook

v1.03:
  jmlrbook.cls

  * Added patch to combnat

  jmlr.cls

  * Added \editors, \editorname and \editorsname

v1.02:
  jmlrbook.cls:

  * Added \issue

  jmlr.cls

  * Added \jmlrissue

v1.01 :

  jmlrbook.cls: 

  * added \importpaper

  * added \titlebody, \SetTitleElement and \IfTitleElement to 
    make it easier to customise the front page of the book.

  jmlr.cls:

  * fixed the last page anchor.

v1.0 : Initial release


==> bit_da_third_place.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{img/bit_da_framework.pdf}
    \caption{PICO++. A student-teacher framework, where the teacher is updated using EMA. The teacher then is used as a target data pseudo-labeler for both supervised contrastive and cross-entropy losses. Details are in Appendix \ref{sec:app_pico}. \vspace{-10pt}}
    \label{fig:pico++}
\end{figure}

\noindent\textbf{Overview:} PICO++ is a variant of  SePiCo \cite{xie2023sepico}. The method composes a student-teacher architecture with learning signals from  semi-supervised contrastive and semi-supervised cross-entropy losses.  The student updates the teacher with EMA, while the teacher provides pseudo-labels for the student network to learn from target data. The samples are constrasted against class prototypes, which are computed from teacher representations. Different from other solutions, the contrastive loss provides explicit source-target domain alignment. Similar to other winning solutions,  PICO++ is built on top of the very strong DAFormer\cite{hoyer2022daformer} architecture. The EMA update provides an implicit ensembling, which has been  shown to improve domain generalization performance \cite{}. 
\newline
\newline
\noindent\textbf{Results: }Source-only and domain adaptation results of PICO++ are reported in Table \ref{tab:baseline_results_new}. PICO++ achieves substantial performance gains compared to the source-only method. 
In Tables \ref{table:zerov2_class_val} and \ref{table:zerov2_class_test} , results are broken into different types of waste. The gain is much greater for classes like rigid plastic and metal, implying that PICO++ has more potential in recognizing classes featuring a relatively regular shape. Nonetheless, a consistent improvement could be observed from all valid classes, showing the effectiveness of PICO++.
\newline
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{ l | c c c c c | c }
            \toprule[1.2pt]
            Method & \rotatebox{0}{background} & \rotatebox{0}{rigid plastic} & \rotatebox{0}{cardboard} & \rotatebox{0}{metal} & \rotatebox{0}{soft plastic} & mIoU \\
            \midrule
            Source-only & 86.87 & 20.11 & 58.32 & 15.7 & 49.36 & 46.07 \\
            PICO++ & 86.10 & 42.77 & 58.79 & 32.13 & 52.33 & 54.43 \\
            \bottomrule[1.2pt]
        \end{tabular}
    }
    \caption{mIoU on ZeroWaste $\rightarrow$ ZeroWasteV2 \textbf{validation} set.}
    \label{table:zerov2_class_val}
\end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{ l | c c c c c | c }
            \toprule[1.2pt]
            Method & \rotatebox{0}{background} & \rotatebox{0}{rigid plastic} & \rotatebox{0}{cardboard} & \rotatebox{0}{metal} & \rotatebox{0}{soft plastic} & mIoU \\
            \midrule
            Source-only & 91.80 & 25.03 & 61.60 & 15.51 & 42.15 & 47.22 \\
            PICO++ & 91.36 & 44.35 & 61.71 & 31.24 & 43.25 & 54.38 \\
            \bottomrule[1.2pt]
        \end{tabular}
    }
    \caption{mIoU on ZeroWaste $\rightarrow$ ZeroWasteV2 \textbf{test} set.}
    \label{table:zerov2_class_test}
\end{table*}
% This section should contain the source-only and domain adaptation results of your team's method on ZeroWaste V2 validation and test sets, including the class-wise results. Optionally, you can include the ablation study results if your method proposes multiple modifications to the baseline. Please elaborate here why you think certain modifications improved segmentation quality.

%\noindent\textbf{Student and Teacher Network Architectures:} The student and teacher networks are identical in architecture; they are built on top of the very strong DAFormer architecture, which is also used as a baseline for the challenge.Additionally, an extra projection head is added to reduce dimensionality (512$\rightarrow$256) for both the student and teacher. During training, the student is updated with loss gradients while the teacher is update with an exponential moving average (EMA)~\citep{} of student iterates. 
%\newline
%\noindent\textbf{Cross-Entropy Losses:} There are two cross-entropy losses used to update the student network. The first is a standard cross entropy loss applied on (augmented) source samples, denoted as $\mathcal{L}_{ce}^s$. Then, augmented target samples are pseudo-labeled using the teacher network, and then mixed with a source sample, creating mixed image $I_m^a$. The target pseudo-label is also mixed with the source label, creating mixed label $Y_m$. Another cross-entropy loss is applied to the student with the resulting mixed image-label pair $\mathcal{L}_{ce}^m(I_m^a, Y_m)$. The ratio of mixed image predictions whose confidence exceed $\beta$, which is called $\lambda_\beta$, reweights the $\mathcal{L}_{ce}^m$. The final loss on mixed images is $\mathcal{L}_{ssl}^m = \lambda_\beta\mathcal{L}_{ce}^m$. This method follows the DACS~\citep{tranheden2021dacs} methodology and allows for self-training using unlabelled target data. 
%\newline
%\noindent\textbf{Contrastive Losses:} In addition to the cross-entropy losses, a semi-supervised contrastive loss is used following SePiCo \cite{}. First, the training is warm-started using cross-entropy losses for $T_w = 3000$ iterations. Then, using the source data, per-label gaussians are fit to teacher projection-head features. These per-label gaussians are used to create proto-types to contrast the student features against. For a single sample of class $i$, the contrastive loss is formulated as 
%    \begin{align}
 %       \mathcal{L}_{cl}^{q_i} = -\log\left[\frac{exp(\frac{q_i^\top \mu_i}{\tau} + \frac{q_i^\top \Sigma_i q_i}{2\tau^2})}{exp(\frac{q_i^\top \mu_i}{\tau} + \frac{q_i^\top \Sigma_i q_i}{2\tau^2}) + \sum_{k=1, k\neq i}^{C}exp(\frac{q_i^\top \mu_k}{\tau} + \frac{q_i^\top \Sigma_k q_i}{2\tau^2})}\right] + \frac{q_i^\top\Sigma_iq_i}{2\tau^2}\,,
  %  \end{align}%
%where $q_i$ represents a query feature $q$ of $i^{th}$ class, and $C$ is the class number, $\tau$ denotes the smoothing factor common in contrastive learning. $\mu_i$ and $\Sigma_i$ are the mean and covariance of the distribution within the prototype from $i^{th}$ class. For source samples, ground truth class labels. For target samples, pseudo-labels are used. This contrastive loss ensures cross-domain feature alignment. For the derivation of this loss, please see the SePiCo paper, section 3.3.2.. Finally the regularization term is formulated as:

%    \begin{align}
%        \mathcal{L}_{reg}^{\bar{q}} = \frac{1}{C\log C} \sum_{k=1}^{C} \log\frac{e^{\bar{q}^{\top} \mu_k/\tau}}{\sum_{l=1}^{K} e^{\bar{q}^\top \mu_l/\tau}}\,,
%    \end{align}%
%where $\bar{q}$ is the average of all features for either source or target domain. This prevents collapse of unsupervised samples. 
%\newline
%\noindent\textbf{Overall loss and Results:} Overall, PICO++ trained with the following objective:

%    \begin{align}
%        \mathcal{L} = \mathcal{L}_{ce}^s + \mathcal{L}_{ssl}^m + \lambda_{cl}\mathcal{L}_{cl} + \lambda_{reg}\mathcal{L}_{reg}
%    \end{align}%
%where $\lambda_{cl}$ and $\lambda_{reg}$ are constant weights.

%As seen in Table 1, this methodology substantially improves over the source-only baseline. 

